Structured Denoising Diffusion Models in Discrete State-Spaces

Denoising diffusion probabilistic models (DDPMs) (Ho et al. 2020) have shown impressive results on image and waveform generation in continuous state spaces. Here, we introduce Discrete Denoising Diffusion Probabilistic Models (D3PMs), diffusion-like generative models for discrete data that generalize the multinomial diffusion model of Hoogeboom et al. 2021, by going beyond corruption processes with uniform transition probabilities. This includes corruption with transition matrices that mimic Gaussian kernels in continuous space, matrices based on nearest neighbors in embedding space, and matrices that introduce absorbing states. The third allows us to draw a connection between diffusion models and autoregressive and mask-based generative models. We show that the choice of transition matrix is an important design decision that leads to improved results in image and text domains. We also introduce a new loss function that combines the variational lower bound with an auxiliary cross entropy loss. For text, this model class achieves strong results on character-level text generation while scaling to large vocabularies on LM1B. On the image dataset CIFAR-10, our models approach the sample quality and exceed the log-likelihood of the continuous-space DDPM model.

==> Tables/toy_results.tex <==
\begin{table}[h!]
  \caption{Quantitative results on toy sequence dataset (sequences .}
  \label{tab:toy}
  \small
  \centering
  \begin{tabular}{lll}
    \toprule
    % \multicolumn{2}{c}{Part}                   \\
    % \cmidrule(r){1-2}
    Model & Model steps & NLL (nats/sequence) ($\downarrow$)\\
    \midrule
    Uniform diffusion & $64$  & $\leq 12.26$  \\
    Mask diffusion & $64$ & $\leq 9.355$ \\
    Gaussian ordinal diffusion & $64$ & $\leq 6.449$ \\
    \bottomrule
  \end{tabular}
\end{table}


==> example_text/old_completion.tex <==

\begin{lstlisting}
T: unas are a small club , " he said . 19 , spent time on the stationary bike this week , but didn 't participate in 11-on-11 drills . Caterpillar is eager to expand in Asia , where it trails local competitors such as Komatsu Ltd ( 6301.T : Quote , Profile , Research ) , and as a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
N: unas are a small club , " he said . 19 , spent time on the stationary bike this week , but didn 't participate in[MASK][MASK]on-11 drills . Caterpillar is eager to expand in[MASK] ,[MASK] it[MASK]s local competitors such as Komatsu Ltd ( 6301.T : Quote [MASK][MASK]e , Research ) , and[MASK] a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
R: unas are a small club , " he said . 19 , spent time on the stationary bike this week , but didn 't participate in 2-on-11 drills . Caterpillar is eager to expand in China , where it faces local competitors such as Komatsu Ltd ( 6301.T : Quote , Profile , Research ) , and as a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
========== 13 ==========
T: unas are a small club , " he said . 19 , spent time on the stationary bike this week , but didn 't participate in 11-on-11 drills . Caterpillar is eager to expand in Asia , where it trails local competitors such as Komatsu Ltd ( 6301.T : Quote , Profile , Research ) , and as a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
N: unas are a small club ,[MASK]" he said . 19 , spent time on the stationary bike this week , but didn 't participate in[MASK][MASK]on-11 drills . Caterpillar is eager to expand in[MASK] ,[MASK] it[MASK]s local competitors such as Komatsu Ltd ( 6301.T : Quote [MASK][MASK]e , Research ) , and[MASK] a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
R: unas are a small club , " he said . 19 , spent time on the stationary bike this week , but didn 't participate in 2-on-11 drills . Caterpillar is eager to expand in China , where it faces local competitors such as Komatsu Ltd ( 6301.T : Quote , Profile , Research ) , and as a slowdown in the U.S. economy dampens the outlook for construction equipment demand in its home market . Merchants along
\end{lstlisting}

\begin{lstlisting}
T: Karrada Street , the main artery of an affluent retail district , said the area has become a virtual shooting gallery for armed guards traveling in sport-utility vehicles . He said he also has asked prosecutors to open a separate investigation . In this case , amid a massive push for increased home ownership , the Fed decided not to intervene . After the vote , Masanori Miyahara , chief counselor of Japan 's Fisheries Agency , said pressure would be on his country and others who depend on the Atlantic
N: [MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK]y[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] become[MASK][MASK] shooting[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] in[MASK][MASK]ut[MASK][MASK][MASK][MASK][MASK][MASK][MASK] also[MASK] [MASK][MASK][MASK][MASK][MASK] a[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] amid[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] not[MASK][MASK][MASK][MASK] After[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] of Japan[MASK][MASK][MASK][MASK][MASK][MASK][MASK], said pressure[MASK][MASK][MASK][MASK][MASK][MASK][MASK] who[MASK][MASK][MASK] Atlantic
R: orism on our list . Plenty of stories are becoming friends . Kwar D 's become a dangerous shooting victim. old families Same for every one in Beirut . The against them are also a terrifying consequence of a long-running taxation process switched sides amidst private expressions of opposition from Berliners as employee numbers do not go public . After the Prime Minister had warned that a " chess like Auction of Japan " would spark a crisis , said pressure group feudal Liberals , who are across the Atlantic
========== 106 ==========
T: Karrada Street , the main artery of an affluent retail district , said the area has become a virtual shooting gallery for armed guards traveling in sport-utility vehicles . He said he also has asked prosecutors to open a separate investigation . In this case , amid a massive push for increased home ownership , the Fed decided not to intervene . After the vote , Masanori Miyahara , chief counselor of Japan 's Fisheries Agency , said pressure would be on his country and others who depend on the Atlantic
N: [MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK]y[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] become[MASK][MASK] shooting[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] in[MASK][MASK]ut[MASK][MASK][MASK][MASK][MASK][MASK][MASK] also[MASK] [MASK][MASK][MASK][MASK][MASK] a[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] amid[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] not[MASK][MASK][MASK][MASK] After[MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK][MASK] of Japan[MASK][MASK][MASK][MASK][MASK][MASK][MASK], said pressure[MASK][MASK][MASK][MASK][MASK][MASK][MASK] who[MASK][MASK][MASK] Atlantic
R: orism on our list . Plenty of stories are becoming friends . Kwar D 's become a dangerous shooting victim. old families Same for every one in Beirut. teams up against them are also equivalent rogues out of a old-fashioned surname amid gargantled opposition from Berliners as a loud and not so sweet . After seeming apparent from the hearing that a sale were under way , John Hatcher of Japanan Uni , Thailand , said pressure on Palau officials , who are in the Atlantic
\end{lstlisting}


==> sections/checklist.tex <==
\section*{Checklist}


\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{sec:discussion}}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See Section \ref{sec:discussion}}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerNo{The code cannot be made available at this time, but we will work to get it open sourced for a camera ready version.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{The training details can be found in Appendix~\ref{sec:appendix_experiments}.}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{We have included averages and standard deviations for as many models as possible for two seeds.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Appendix~\ref{sec:appendix_experiments}.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We have included citations to all datasets.}
  \item Did you mention the license of the assets?
    \answerNA{These are standard datasets.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNo{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{} While it is valid to question if such information appears in large datasets like CIFAR-10 and LM1B, these are standard benchmarks, and it is beyond the scope of this work to do a thorough analysis.
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

